Automatic Verification of Erlang-Style Concurrency

This paper presents an approach to verify safety properties of Erlang-style, higher-order concurrent programs automatically. Inspired by Core Erlang, we introduce Lambda-Actor, a prototypical functional language with pattern-matching algebraic data types, augmented with process creation and asynchronous message-passing primitives. We formalise an abstract model of Lambda-Actor programs called Actor Communicating System (ACS) which has a natural interpretation as a vector addition system, for which some verification problems are decidable. We give a parametric abstract interpretation framework for Lambda-Actor and use it to build a polytime computable, flow-based, abstract semantics of Lambda-Actor programs, which we then use to bootstrap the ACS construction, thus deriving a more accurate abstract model of the input program. We have constructed Soter, a tool implementation of the verification method, thereby obtaining the first fully-automatic, infinite-state model checker for a core fragment of Erlang. We find that in practice our abstraction technique is accurate enough to verify an interesting range of safety properties. Though the ACS coverability problem is Expspace-complete, Soter can analyse these verification problems surprisingly efficiently.

==> macros.tex <==
% !TEX root = main.tex
\makeatletter

\def\my@test@bf{bx}

\newcommand{\Soter}{\textsf{Soter}}
\newcommand{\SoterUrl}{\url{http://mjolnir.cs.ox.ac.uk/soter/}}
\newcommand{\BFC}{{BFC}}
\newcommand{\Lang}{%
	\texorpdfstring%
        {${{\ifx\f@series\my@test@bf\boldsymbol{\lambda}\else\lambda\fi}{\textsc{\scriptsize Actor}}}$}%
		{Lambda-Actor}%
}


\mathchardef\breakingcomma\mathcode`\,
{\catcode`,=\active
  \gdef,{\breakingcomma\discretionary{}{}{}}
}
\newcommand{\commabr}[1]{\mathcode`\,=\string"8000 #1}

\newcommand\textbfit[1]{{\bf \emph{#1}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Generic Math operators and abbreviations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\bigO}[1]{\ensuremath{O(#1)}}

\let\vect\vec
\renewcommand{\vec}[1]{\mathbf{#1}}
\newcommand{\sem}[1]{\llbracket#1\rrbracket}

\newcommand{\Nat}{\mathbb{N}}
\newcommand{\Int}{\mathbb{Z}}
\newcommand{\powerset}{\mathscr{P}}
\newcommand{\finpow}{\powerset_{\!\!f}}
\newcommand{\union}{\cup}
\newcommand{\inters}{\cap}
\newcommand{\Union}{\bigcup}
\newcommand{\Inters}{\bigcap}
\newcommand{\dunion}{\uplus}
\newcommand{\Dunion}{\biguplus}
\providecommand{\implies}{\Rightarrow}
\newcommand{\iif}{\Leftrightarrow}
\newcommand{\iso}{\cong}

\newcommand{\freevars}{\operatorname{fv}}

\newcommand{\tuple}[1]{\langle\commabr{#1}\rangle}
\newcommand{\lst}[3][1]{{#2_{#1}}\ldots {#2_{#3}}}    % b_a ... b_c
\newcommand{\lstc}[3][1]{\commabr{{#2_{#1}},\ldots, {#2_{#3}}}} % b_a ,..., b_c
\newcommand{\lsts}[4]{#1_#2#4\ldots#4 #1_{#3}}        % b_a d...d b_c
\newcommand{\vct}[3][]{\ensuremath{\bar #2}} % unused args are intentional so \vect can be redef to be \lst

\newcommand{\is}{\mathrel{\mathop:}=}
\newcommand\makeset[1]{{ {\{} #1{\}} }}
\newcommand\sendto[2]{{#2 \mathbin{\hbox{!}} #1}}
\newcommand\receivefrom[2]{{#2 \mathbin{\hbox{?}} #1}}

%%% Parametric extendible arrow %%%

\newcommand{\xRightarrow}[2]{%
  \ext@arrow3399{\longrightarrowtfill@}{#1}{#2}}
\newcommand{\longrightarrowtfill@}{%
  \arrowfill@\Relbar\Relbar\Rightarrow}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\larg}[2]{#1.\text{arg}_{#2}}
\newcommand{\largn}[1]{\operatorname{arity}(#1)}


\newcommand{\Data}{\dom{Data}}

\newcommand{\Vars}{\mathcal{V}}
\newcommand\order{\operatorname{ord}}
\newcommand\FV{\mathit{FV}}

\newcommand{\Prog}{\ensuremath{\mathcal{P}}}
\newcommand\var{\operatorname{var}}

\newcommand{\rulename}[1]{\textbf{\textit{#1}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ACS abbreviations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\Acs}{\ensuremath{\mathcal{A}}}
\newcommand{\VAS}{\ensuremath{\mathcal{V}}}
\newcommand{\transto}{\mathrel{\rightarrowtail}}

\newcommand{\ecsrule}[4][\pid]{#1\colon #2\xrightarrow{#3}#4}

\def\eTau#1[#2-->#3]{\ecsrule[\ifx!#1!\pid\else #1\fi]{#2}{\tau}{#3}}
\def\eSend#1[#2--#3!#4-->#5]{\ecsrule[\ifx!#1!\pid\else #1\fi]{#2}{#3\mathbin{!}#4}{#5}}
\def\eRec#1[#2--?#3-->#4]{\ecsrule[\ifx!#1!\pid\else #1\fi]{#2}{?#3}{#4}}
\def\eSpawn#1[#2--v#3.#4-->#5]{\ecsrule[\ifx!#1!\pid\else #1\fi]{#2}{\nu#3.#4}{#5}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Erlang semantics
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\fun}{\mathit{fun}}
\newcommand{\pat}{\mathit{pat}}

% Constructs (for out of listing env use)
\newcommand{\Rec}{\erl[columns=fullflexible]{receive}}
\newcommand{\Send}[2]{\erl[columns=fullflexible]{send}(#1, #2)}
\newcommand{\Spawn}[3][]{\erl[columns=fullflexible]{spawn}\ensuremath{_{#1}}\ #2\ #3}
\newcommand{\Self}{\erl[columns=fullflexible]{self}}

% Processes

%% \proc to be used only in informal semantics
\newcommand{\proc}[3]{\tuple{#1}^{#2}_{#3}} % exp pid queue

\newcommand{\pid}{\iota}
\newcommand{\timest}{\vartheta}
\newcommand{\cntr}{t} % contour!

% Generic operations
\newcommand{\cons}{\mathbin{\cdot}}
\newcommand{\eseq}{\ensuremath{\epsilon}}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Abstract Machine
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\dom}[1]{\ensuremath{\mathit{#1}}}
\newcommand{\ProgLoc}{\dom{ProgLoc}}
\newcommand{\Exp}{\dom{Exp}}
\newcommand{\Constr}{\Sigma}
\newcommand{\Val}{\dom{Value}}
\let\Value\Val
\newcommand{\State}{\dom{State}}
\newcommand{\Store}{\dom{Store}}
\newcommand{\ProcState}{\dom{ProcState}}
\newcommand{\Procs}{\dom{Procs}}
\newcommand{\Mailbox}{\dom{Mailbox}}
\newcommand{\Mailboxes}{\dom{Mailboxes}}
\newcommand{\Closure}{\dom{Closure}}
\newcommand{\Env}{\dom{Env}}
\newcommand{\Var}{\dom{Var}}

\newcommand{\TimeStamp}{\dom{TimeSt}}
\newcommand{\Time}{\dom{Time}}
\newcommand{\Contour}{\dom{Time}}
\newcommand{\Pid}{\dom{Pid}}

\newcommand{\Addr}{\dom{Addr}}
\newcommand{\AddrKont}{\dom{KAddr}}
\newcommand{\AddrVar}{\dom{VAddr}}
\let\AddrVal\AddrVar % alias in case of confusion
\newcommand{\Msg}{\ensuremath{\widehat{\dom{Msg}}}}

\newcommand{\Kont}{\dom{Kont}}

\newcommand{\finmap}{\rightharpoonup}
\newcommand{\fundom}{\operatorname{dom}}
\newcommand{\undef}[2]{#1(#2) = \bot}

\newcommand{\match}{\operatorname{match}}

\newcommand{\msg}{\ensuremath{m}}
\newcommand{\mailbox}{\ensuremath{\mathfrak{m}}}
\newcommand{\emptymb}{\ensuremath{\epsilon}}
\newcommand{\emptycntr}{\ensuremath{\epsilon}}

\newcommand{\data}{\delta}
\newcommand{\databot}{\_}

\newcommand{\mailmatch}{\operatorname{mmatch}}
%\newcommand{\enqueue}{\operatorname{enqueue}}
\newcommand{\enqueue}{\operatorname{enq}}
% \newcommand{\newKaddr}{\operatorname{new}_{ka}}
\newcommand{\newKPush}{\operatorname{new}_{\text{kpush}}}
\newcommand{\newKPop}{\operatorname{new}_{\text{kpop}}}
\newcommand{\newVaddr}{\operatorname{new}_{\text{va}}}
\newcommand{\newpid}{\operatorname{new}_{\text{pid}}}
\let\newPid\newpid
\newcommand{\tick}{\operatorname{tick}}

\newcommand{\kont}{\ensuremath{\kappa}}
\newcommand{\kontTag}[1]{\text{\sffamily #1}}
\newcommand{\kontData}[2]{\kontTag{#1}\tuple{#2}}
\newcommand{\kTop}{\text{\sffamily Stop}}
\let\kStop\kTop % unfortunate choice of macro name
\newcommand{\kArg}[1]{\kontData{Arg$_{#1}$}}
\newcommand{\kCase}{\kontData{Case}}

\newcommand{\resolve}[1][]{\operatorname{res}_{#1}}
\newcommand{\absresolve}[1][]{\widehat{\operatorname{res}}_{#1}}

\newcommand{\CFA}[1]{\mbox{#1-CFA}}
\newcommand{\zCFA}{\CFA{0}}
\newcommand{\kCFA}{\CFA{$k$}}
\newcommand{\kwCFA}{\textup{CFA($k$,$w$)}}

\newcommand{\semTo}{\to}
\newcommand{\cfaTo}{\leadsto}
\newcommand{\acsTo}{\to_{{\textup{acs}}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Abstract Interpretation
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\AbsInt}{\mathcal{I}}
\newcommand{\DataAbs}{\mathcal{D}}
\newcommand{\TimeAbs}{\mathcal{T}}
\newcommand{\MailboxAbs}{\mathcal{M}}
\newcommand{\MsgAbs}{\mathcal{D}_{\text{msg}}}

\newcommand{\leqmb}[1][m]{\leq_{\text{#1}}}
\newcommand{\leqx}[1][]{\leq_{\text{#1}}}
\newcommand{\id}{\text{id}}
% ABS
%% Might style notation
\gdef\abs#1{\ifx\to#1\cfaTo\else\widehat#1\fi}
%% Cousot style notation
% \gdef\abs#1{\ifx\to#1\cfaTo\else{{#1}^{\sharp}}\fi}
%% Tilde notation
% \gdef\abs#1{\ifx\to#1\cfaTo\else\widetilde#1\fi}


\newcommand{\join}{\sqcup}
\newcommand{\bigjoin}{\bigsqcup}

\newcommand{\absf}[1][]{\alpha_{\text{#1}}}
\newcommand{\concf}[1][]{\gamma_{\text{#1}}}
\newcommand{\absfp}[1][ACS]{\alpha^{\text{pat}}_{\text{#1}}}
\newcommand{\absfK}[1][ACS]{\alpha^{k}_{\text{#1}}}

\newcommand{\hole}{\_}
\newcommand{\depthD}[2][D]{{\lfloor{#2}\rfloor}_{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Complexity classes
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\complclass}{\textsc}
\newcommand{\expspace}{\complclass{Expspace}}
\newcommand{\exptime}{\complclass{Exptime}}
\newcommand{\ptime}{\complclass{P}}
\newcommand{\pspace}{\complclass{Pspace}}
\newcommand{\np}{\complclass{NP}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Typesetting of operational semantic tables
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newlength{\colwd}

\newcommand{\CondCell}[2][if]{%
	\parbox[t]{\colwd}{#1\space$\begin{array}[t]{@{}r@{\;}l@{}}#2\end{array}$}}

\newcommand{\ResCell}[2][then]{%
	\parbox[t]{\colwd}{#1\space$\begin{array}[t]{@{}r@{\;}l@{}}#2\end{array}$}}

\newcounter{RULE}
\newcommand{\formatRuleName}[1]{\textbf{\small #1}}
\newcommand{\RuleName}[1]{%
	\formatRuleName{#1}%
	\renewcommand{\theRULE}{\formatRuleName{#1}}%
	\refstepcounter{RULE}%
}

\newcommand{\ARN}[1]{Abs#1}
\newcommand{\AbsRuleName}[1]{%
	\smallskip%
	\formatRuleName{\ARN{#1}}%
	\renewcommand{\theRULE}{\formatRuleName{\ARN{#1}}}%
	\refstepcounter{RULE}%
}

\newcommand{\RulesSection}[1]{\textbf{\color{red!40!black}#1}}

\newcommand{\atom}[1]{\text{\texttt{\color{atom}#1}}}

\newcommand{\StopAddr}{\boldsymbol{\ast}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Syntax environment
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begingroup
\catcode`\|=\active%
\gdef\@redefbar{%
    \catcode`\|=\active%
    \def|{\hspace{3pt}\mid\hspace{3pt}}
}
\endgroup

\newenvironment{syntax}{%
    \begin{equation*}
    \def\prod{\mathrel{::=}}
    \renewcommand{\arraystretch}{1.2}
    \@redefbar
    \begin{array}{rl}%
}
{%
    \end{array}
    \end{equation*}
}
\let\grammar\syntax
\let\endgrammar\endsyntax

\makeatother

